Arabic Offensive Language on Twitter: Analysis and Experiments

Detecting offensive language on Twitter has many applications ranging from detecting/predicting bullying to measuring polarization. In this paper, we focus on building a large Arabic offensive tweet dataset. We introduce a method for building a dataset that is not biased by topic, dialect, or target. We produce the largest Arabic dataset to date with special tags for vulgarity and hate speech. We thoroughly analyze the dataset to determine which topics, dialects, and gender are most associated with offensive tweets and how Arabic speakers use offensive language. Lastly, we conduct many experiments to produce strong results (F1 = 83.2) on the dataset using SOTA techniques.

==> classifiers.tex <==
\section{Classification Models}
\label{classifiers}
Some state-of-the-art techniques use complex models to achieve best results. Often the level of complexity of models rises a lot just to achieve small increase in performance. In our suite of systems, we want to have models that are small in size and easy to deploy while providing good results. To this end, we avoid usage of deep learning and contextual embedding models and opt for Supoprt Vector Machines (SVMs) with character n-gram vectors weighted by term frequency-inverse document frequency (tf-idf) as features.
The range of n-gram can influence size of model and its performance. For each component of our suite, we experimented with different ranges of n-gram and calculated model size along with respective performance. Table \ref{tab:size} illustrates this study for offensiveness detection (C[a-b] denotes character n-gram ranging from a to b. P, R and F1 stand for macro-averaged precision, recall and F1 respectively). We can see that going from n-gram range of C[1-3] to C[2-7] increases model size (classifier + vectorizer) from 3.9 MB to 120.5 MB while improving the F1 score by 2.4. Although C[2-7] is a better system, C[1-3] is much more suitable for deployment due to its small size. We perform similar study (omitted here for conciseness) for all modules of ASAD. In deployed version, we use models that are small in size but also achieve good results. Table \ref{tab:allscores} lists performance of modules in deployed version of ASAD on test sets.

\begin{table}[]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|}
        \hline

        \bf{Classifier} & \bf{Features} & \bf{Size (classifier + vectorizer)} & \bf{Acc} & \bf{P} & \bf{R} & \bf{F1} \\ \hline
        SVM & C[1-3] & 3.9 MB & 91.15 &	88.77 &	82.36 &	85.03\\
        SVM & C[2-4] & 14.5 MB &	91.55 &	89.17 &	83.36 &	85.83\\
        SVM & C[2-5] & 37.5 MB &	92.00 &	89.07	& 85.13	& 86.90\\
        SVM & C[2-6] & 73.35 MB	& 91.75	& 87.57	& 86.37	& 86.95\\
        SVM & C[2-7] & 120.5 MB &	91.80 &	86.86	& 88.07	& 87.44\\
        
        \hline
        
    \end{tabular}
    \caption{Comparison of size vs performance on offensiveness detection}
    \label{tab:size}
\end{table}


\begin{table}[]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|}
        \hline

        \bf{Module} & \bf{Classifier} & \bf{Features} & \bf{Acc} & \bf{P} & \bf{R} & \bf{F1-score} \\ \hline
        Offensiveness & SVM & C[1-3] & 91.15	& 88.77 &	82.36 &	85.03\\
        Hate Speech & SVM & C[2-4] & 79.77 &	74.72 &	72.18 &	73.22\\
        Sentiment & SVM & C[1-3] & 75.53	& 74.58 &	73.18 &	73.67\\
        Adult Content & SVM & C[1-3] & 95.39 &	91.93 &	85.79 &	88.52\\
        Spam & SVM & C[1-3] & 99.43	& 99.39	& 97.28 &	98.31\\
        Dialect ID & SVM & C[2-4] & 54.47	& 60.90 &	54.59 &	54.13\\
        \hline
        
    \end{tabular}
    \caption{Performance of different components of ASAD}
    \label{tab:allscores}
\end{table}
